Performance Tuning of Hadoop MapReduce: A Noisy Gradient Approach

Hadoop MapReduce is a framework for distributed storage and processing of large datasets that is quite popular in big data analytics. It has various configuration parameters (knobs) which play an important role in deciding the performance i.e., the execution time of a given big data processing job. Default values of these parameters do not always result in good performance and hence it is important to tune them. However, there is inherent difficulty in tuning the parameters due to two important reasons - firstly, the parameter search space is large and secondly, there are cross-parameter interactions. Hence, there is a need for a dimensionality-free method which can automatically tune the configuration parameters by taking into account the cross-parameter dependencies. In this paper, we propose a novel Hadoop parameter tuning methodology, based on a noisy gradient algorithm known as the simultaneous perturbation stochastic approximation (SPSA). The SPSA algorithm tunes the parameters by directly observing the performance of the Hadoop MapReduce system. The approach followed is independent of parameter dimensions and requires only $2$ observations per iteration while tuning. We demonstrate the effectiveness of our methodology in achieving good performance on popular Hadoop benchmarks namely \emph{Grep}, \emph{Bigram}, \emph{Inverted Index}, \emph{Word Co-occurrence} and \emph{Terasort}. Our method, when tested on a 25 node Hadoop cluster shows 66\% decrease in execution time of Hadoop jobs on an average, when compared to the default configuration. Further, we also observe a reduction of 45\% in execution times, when compared to prior methods.

==> algo.tex <==
\begin{algorithm}
\caption{Simultaneous Perturbation Stochastic Approximation}
\label{algo}
\begin{algorithmic}[1]
\STATE Let initial parameter setting be $\theta_0\in X\subset\R^n$
\FOR{$n=1,2\ldots,N$}
\STATE Observe the performance of system $f(\theta_n)$.
\STATE Generate a random perturbation vector $\Delta_n \in\R^n$.
\STATE Observe the performance of system $f(\theta_n+\delta\Delta_n)$.
\STATE Compute the gradient estimate $\hat{\nabla} f_n(i)=\frac{f(\theta_n+\delta \Delta_n)-f(\theta_n)}{\delta\Delta_n(i)}.$\label{gres}
\STATE Update the parameter in the negative gradient direction $\theta_{n+1}(i)=\Gamma\big(\theta_n(i)-\alpha_n\frac{f(\theta_n+\delta\Delta_n)-f(\theta_n)}{\delta\Delta(i)}\big)$.\label{update}
\ENDFOR
\RETURN $\theta_{N+1}$
\end{algorithmic}
\label{politer}
\end{algorithm}

==> benchProfile.tex <==
\begin{figure*}
  \makebox[\linewidth][c]{
\begin{subfigure}[b]{.33\linewidth}
\centering
\includegraphics[width=.9\textwidth]{imagena.jpg}
\caption{Convergence in Terasort}
\end{subfigure}%

\begin{subfigure}[b]{.33\linewidth}
\centering
\includegraphics[width=.9\textwidth]{imagena.jpg}
\caption{Convergence in WordCount}
\end{subfigure}%

\begin{subfigure}[b]{.33\linewidth}
\centering
\includegraphics[width=.9\textwidth]{imagena.jpg}
\caption{Convergence in Grep}
\end{subfigure}%
  }
  \\\\
    \makebox[\linewidth][c]{
\begin{subfigure}[b]{.33\linewidth}
\centering
\includegraphics[width=.9\textwidth]{imagena.jpg}
\caption{Convergence in Bigram Count}
\end{subfigure}%

\begin{subfigure}[b]{.33\linewidth}
\centering
\includegraphics[width=.9\textwidth]{imagena.jpg}
\caption{Convergence in Inverted Index}
\end{subfigure}%
  }
  
  \caption{Profile of Benchmarks. CPU, Memory and Network Usage (monitored usign Ganglia[ref])}
  \label{fig:benchProfile}
\end{figure*}
